Breaking the Communication-Privacy-Accuracy Trilemma

Two major challenges in distributed learning and estimation are 1) preserving the privacy of the local samples; and 2) communicating them efficiently to a central server, while achieving high accuracy for the end-to-end task. While there has been significant interest in addressing each of these challenges separately in the recent literature, treatments that simultaneously address both challenges are still largely missing. In this paper, we develop novel encoding and decoding mechanisms that simultaneously achieve optimal privacy and communication efficiency in various canonical settings. In particular, we consider the problems of mean estimation and frequency estimation under $\varepsilon$-local differential privacy and $b$-bit communication constraints. For mean estimation, we propose a scheme based on Kashin's representation and random sampling, with order-optimal estimation error under both constraints. For frequency estimation, we present a mechanism that leverages the recursive structure of Walsh-Hadamard matrices and achieves order-optimal estimation error for all privacy levels and communication budgets. As a by-product, we also construct a distribution estimation mechanism that is rate-optimal for all privacy regimes and communication constraints, extending recent work that is limited to $b=1$ and $\varepsilon=O(1)$. Our results demonstrate that intelligent encoding under joint privacy and communication constraints can yield a performance that matches the optimal accuracy achievable under either constraint alone.

==> backup/sec_prior_works_v1.tex <==

\begin{table}[bt!]
\centering
\mbox{}\hfill
\begin{minipage}{.5323\linewidth}
\begin{tabular}{|c|c|c|c|c|}
\hline 
$\vphantom{\Theta \lp \frac{d}{\lp n^2\rp } \rp}$ & Privacy & Comm. & $\ell_2$ error\\ 
\hline 
    Thm.~\ref{thm:mean_estimation} & $\forall\, \varepsilon$ & $\forall\, b $ & $\frac{d}{n\min\lp \varepsilon^2, \varepsilon, b \rp}$ \vphantom{$\lp \frac{d}{n\min\lp \varepsilon^2, \varepsilon, b \rp}\rp$}\\% & public-coin\\
\hline 
   Cp\cite{g2019vqsgd} & $\varepsilon \succeq 1$ & $b \succeq \log d$ & $\frac{d^2}{n}$ \vphantom{$\lp \frac{d^2}{n}\rp$}\\%& private-coin \\
\hline
      Sp \cite{g2019vqsgd} & $\varepsilon \succeq \log d$ & $b \succeq \log d$ & $\frac{d}{n}$ \vphantom{$\lp \frac{d^2}{n}\rp$}\\%& private-coin \\
\hline
\end{tabular}
\caption{Comparison between our mean estimation scheme and vqSGD \cite{g2019vqsgd},  where Cp and Sp refer to the Cross-polytope and Simplex  methods in \cite{g2019vqsgd}. Our scheme applies to general communication and privacy regimes, and achieves optimal estimation error for all scenarios.} \label{tbl:mean_est}
\end{minipage} \hfill
\begin{minipage}{.4505\linewidth}
\begin{tabular}{|c|c|c|}
\hline 
$\vphantom{\Theta \lp \frac{d}{\lp n^2\rp } \rp}$ 
Privacy
& $\varepsilon \in (0, 1)$ & $\varepsilon \in \lp 1, \log d\rp$  \\
\hline $\vphantom{\Theta \lp \frac{d}{n \min{\lp e, \lp e-1\rp^2, 2\rp}} \rp}$
    SS \cite{ye2017optimal} 
    & \cellcolor{OrangeRed!40}$d$ bits 
    & \cellcolor{OrangeRed!40}$ \max\lp \frac{d}{e^\varepsilon}, \log d \rp$%\footnote{The exact $k$-SS requires communicating $\log {n \choose w}$ bits, where $w = \lceil d/e^\varepsilon +1 \rceil$.} %bits 
    \\
\hline $\vphantom{\Theta \lp \frac{d}{n \min{\lp e, \lp \varepsilon-1\rp, 2\rp}} \rp}$
    HR\cite{acharya2019hadamard} 
    & \cellcolor{OrangeRed!40}$\log d$ bits 
    & \cellcolor{OrangeRed!40}$\log d$ bits 
    \\
\hline $\vphantom{\Theta \lp \frac{d}{n \min{\lp e, \lp \varepsilon-1\rp, 2\rp}} \rp}$
    $1$-HR\cite{acharya2019communication} 
    & \cellcolor{CornflowerBlue!40} $1$ bit
    & -
    \\
\hline $\vphantom{\Theta \lp \frac{d}{n \min{\lp e, \lp \varepsilon-1\rp, 2\rp}} \rp}$
    Thm.~\ref{thm:dist_estimation}
    & \cellcolor{CornflowerBlue!40}$1$ bit
    & \cellcolor{CornflowerBlue!40}$\min\lp \lceil \varepsilon \rceil,\log d \rp$ 
    \\
\hline
\end{tabular}
    \caption{Comparison between LDP distribution estimation schemes. Under same privacy guarantee, our scheme is more communication efficient while achieves same accuracy.} \label{tbl:dist_compare}
\end{minipage}
\end{table}

\begin{table}[b!]
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline 
$\vphantom{\Theta \lp \frac{d}{\lp n^2\rp } \rp}$
& Loss & Estimation error & Communication\\
%\hline 
%    Heavy hitter \cite{Bassily2017} 
%    & $\ell_\infty$ 
%    & $\Theta\lp \sqrt{\frac{\log d}{n \varepsilon^2}} \rp$ ($\varepsilon = O(1)$) 
%    & $1$ bit \\

\hline 
    OUE \cite{wang2017locally} 
    & $\ell_2$ 
    & $\Theta \lp\frac{d}{n \min \lp \lp e^\varepsilon -1 \rp^2, e^\varepsilon\rp} \rp$ 
    & $d$ bits \\
\hline 
    Thm~\ref{thm:emp_dist_estimation} 
    & $\ell_2$ 
    & $\Theta\lp \frac{d}{n \min \lp \lp e^\varepsilon -1 \rp^2, e^\varepsilon\rp} \rp$ 
    & $\min\lp\lceil \varepsilon \rceil,\log d\rp$ bits \\
\hline $\vphantom{\Theta \lp \sqrt{\frac{d^2}{n \min{\lp e^\varepsilon, \lp e^\varepsilon-1\rp^2, 2^b\rp}}} \rp}$
     Thm.~\ref{thm:emp_dist_estimation} (Heavy hitter)
    & $\ell_\infty$ 
    & $ \Theta \lp\sqrt{\frac{\log d}{n \min \lp \varepsilon, \varepsilon^2 \rp}} \rp$ 
    & $\lceil \varepsilon \rceil$ bits \\    
%\hline 
%   Theorem.~\ref{thm:emp_dist_estimation}
%    & $\ell_1$ 
%    & $\Theta\lp \sqrt{\frac{d^2}{n \min \lp \lp e^\varepsilon -1 \rp^2, e^\varepsilon\rp}} \rp$ 
%    & $O(\lceil \varepsilon \rceil)$ bits \\
\hline
\end{tabular}
\caption{Comparison of different frequency estimation schemes.} \label{tbl:emp_est}
\end{center}
\end{table}
%\newpage


Previous works in the mean estimation problem \cite{an2016distributed, alistarh17qsgd, wen2017terngrad, wang2018atomo, g2019vqsgd,barnes2020rtopk} mainly focus on reducing communication cost, for instance, by random rotation \cite{an2016distributed} and sparsification \cite{alistarh17qsgd, wen2017terngrad, wangni2018gradient, braverman2016communication}. Among them, \cite{g2019vqsgd} considers LDP simultaneously. It proposes vector quantization and takes privacy into account, developing a scheme for $\varepsilon = \Theta(1)$ and $b = \Theta(\log d)$ with estimation error $O(d^2/n)$. In contrast, the scheme we develop in Theorem~\ref{thm:mean_estimation} achieves an estimation error $O(d/n)$ when $\varepsilon=\Theta(1)$ and $b = \Theta(\log d)$. Moreover, our scheme is applicable for any $\varepsilon$ and $b$ and achieves the optimal estimation error, which we show by proving a matching information theoretic lower bound. A key step in our scheme is to pre-process the local data via Kashin's representation \cite{lyubarskii2010uncertainty}. While various compression schemes, based on quantization, sparsification and dithering have been proposed in the recent literature and Kashin's representation for communication efficiency has been also explored in a few works \cite{fuchs2011spread, studer2012signal, caldas2018expanding, safaryan2020uncertainty}, it is particularly powerful in the case of joint communication and privacy constraints as it helps spread the information in a vector evenly in every dimension. This helps mitigate the error due to subsequent noise introduced by privatization and compression. See Table~\ref{tbl:mean_est} for a comparison of our results with \cite{g2019vqsgd}.

The recent works of \cite{nguyn2016collecting, wang2019locally} also consider estimating empirical mean under $\varepsilon$-LDP. They show that if the data is from $d$-dimensional unit $\ell_\infty$ ball, i.e. $X_i \in [-1, 1]^d$, then directly quantizing, sampling and perturbing each entry can achieve optimal $\ell_\infty$ estimation error that matches the LDP lower bound in \cite{duchi2013local}. Nevertheless, their approach does not yield good $\ell_2$ error in general. Indeed, as in the case of separation schemes discussed in Section~\ref{sec:separation_is_suboptimal}, the $\ell_2$ error of their scheme can grow with $d^2$. We emphasize that in many applications the $\ell_2$ estimation error (i.e. MSE) is a more appropriate measure than $\ell_\infty$. For instance, \cite{agarwal2018cpsgd} shows a direct connection between the MSE in mean estimation and the convergence rate of distributed SGD.

Frequency estimation under local differential privacy has been studied in \cite{wang2017locally}, where they propose schemes for estimating the frequency of an individual symbol and minimizing the variance of the estimator. Some of their schemes, while matching the information-theoretic lower bound on $\ell_2$ estimation error under privacy constraints, require large communication. For instance, the scheme Optimal Unary Encoding (OUE) achieves optimal $\ell_2$ estimation error, but the communication required is $O(d)$ bits, which, as we show in this work,  can be reduced to $O(\min(\lceil \varepsilon \rceil,\log d))$ bits. We do this by  developing a new scheme for frequency estimation under joint privacy and communication constraints. We establish the optimality of our proposed schemes by deriving matching information theoretic lower bounds on $r_{\texttt{FE}}\lp \ell_2, \varepsilon, b \rp$.

Frequency estimation is also closely related to heavy hitter estimation \cite{hsu12hh, erlingsson14rappor, Bassily2015, zhan16hh, Bassily2017, bun18hh, acharya2019communication}, where the goal is to discover symbols that appear frequently in a given data set and estimate their frequencies. This can be done if the error of estimating the frequency of each individual symbol can be controlled uniformly (i.e. by a common bound), and thus is equivalent to minimizing the $\ell_\infty$ error of estimated frequencies, i.e. $r_{\texttt{FE}}\lp \ell_\infty, \varepsilon, b \rp$. It is shown in \cite{Bassily2015} that in the high privacy regime $\varepsilon = O(1)$, 
$ r_{\texttt{FE}}\lp \ell_\infty, \varepsilon, b \rp = \Theta( \sqrt{\log d /n \varepsilon^2} ),  $
and this rate can be achieved via a $1$-bit public-coin scheme that has a runtime almost linear in $n$ \cite{Bassily2017}. An extension, which we describe in Section~\ref{proof:freq_l_infty} of the appendix, generalizes the achievability in \cite{Bassily2015} to arbitrary  $\varepsilon$ and $b$, achieving
$ r_{\texttt{FE}}\lp \ell_\infty, \varepsilon, b \rp = O(\sqrt{\log d/n \min{\lp\varepsilon^2, \varepsilon, b\rp}}).$
We compare our scheme and existing results in Table~\ref{tbl:emp_est}.






If we further assume $X^n$ are drawn from some discrete distribution $\bm{p}$, then the problem falls into distribution estimation under local differential privacy \cite{duchi2013local, erlingsson14rappor, wang2016mutual, kairouz16, ye2017optimal, acharya2019hadamard, acharya2019communication} and limited communication \cite{han2018geometric, zhang2013information, garg2014communication, braverman2016communication, han2018distributed, barnes2019lower}. Tight lower bounds are given separately: for instance \cite{ye2017optimal, acharya2019hadamard} shows $r_{\texttt{DE}}\lp \ell_1, \varepsilon, \log d \rp = \Omega(\sqrt{d^2/n\min((e^\varepsilon-1)^2, e^\varepsilon)})$ and \cite{han2018distributed} shows $r_{\texttt{DE}}\lp \ell_1, \infty, b \rp = \Omega(\sqrt{d^2/n 2^b})$. 


We show that these lower bounds can be achieved simultaneously (Theorem~\ref{thm:dist_estimation}). Our result recovers the result of \cite{acharya2019communication} when $b=1$ and  $\varepsilon = O(1)$ as a special case. See %Figure~\ref{fig:dist_est_achievability} and 
Table~\ref{tbl:dist_compare} for a comparison. 





\subsection{Our Contributions and Techniques}
\label{sec:contributions}
To summarize, our main technical contributions include:
\begin{itemize}[leftmargin=1em,topsep=0pt]
     \item For mean estimation, we characterize the optimal $\ell_2$ error $r_{\texttt{ME}} \lp \ell_2\rp = \Theta\lp d/n\min\lp \varepsilon^2, \varepsilon, b \rp \rp$, by designing a public-coin scheme, Subsampled and Quantized Kashin's Response (SQKR), and proving its optimility by deriving matching information theoretic bounds (in Theorem~\ref{thm:mean_estimation}). Our encoding scheme is based on Kashin's representation \cite{lyubarskii2010uncertainty} and random sampling, which allow the server to construct unbiased estimator of each $X_i$ privately and with little communication. This significantly improves on \cite{g2019vqsgd}, which focuses on the special case $\varepsilon = \Omega(1), b = \log d$ and achieves quadratic dependence on $d$ in that case. 
     
    \item For frequency estimation, we characterize the optimal $\ell_1$ and $\ell_2$ errors under both constraints (in Theorem~\ref{thm:emp_dist_estimation}) and propose an order-optimal public-coin scheme called Recursive Hadamard Response (RHR).
    Our result shows that the accuracy is dominated only by the worst-case constraint, and this implies that one can achieve the less stringent constraint for free. The proposed scheme RHR is based on Hadamard transform, but unlike previous works using Hadamard transform, e.g. \cite{Bassily2017}, we crucially leverage the recursive structure of the Hadamard matrix, which allows us to make the estimation error decay exponentially as $\varepsilon$ and $b$ grow. RHR is computationally efficient, and the decoding complexity is $O(n+d\log d)$. We establish its optimality by showing matching lower bounds on the performance.
    
    
    \item We show that RHR easily leads to an optimal scheme for distribution estimation \cite{acharya2019communication, acharya2019hadamard, ye2017optimal}, in which case it does not require shared randomness and achieves order-optimal $\ell_1$ and $\ell_2$ error for all privacy regimes and communication budgets.  We also provide empirical evidence that our scheme requires significantly less communication while achieving the same accuracy and privacy levels as the state-of-the-art approaches. See Section~\ref{sec:exp} for more results.
    
    %\item We show that the scheme we develop for frequency estimation easily leads to an optimal scheme for distribution estimation \cite{acharya2019communication, acharya2018distributed, ye2017optimal}, in which case it does not require shared randomness and achieves order-optimal $\ell_1$ error for all privacy regimes and communication budgets.  We also provide empirical evidence that our scheme requires significantly less communication while achieving the same accuracy and privacy levels as the state-of-the-art approaches. See Section~\ref{sec:exp}.
    
\end{itemize}

\iffalse
\begin{table}[ht]
\begin{minipage}[b]{0.5\linewidth}
\centering
\begin{tabular}{|c|c|c|}
\hline 

Privacy levels
& $\varepsilon \in (0, 1)$ & $\varepsilon \in \lp 1, \log d\rp$  \\
\hline $\vphantom{\Theta \lp \frac{d}{n \min{\lp e, \lp e-1\rp^2, 2\rp}} \rp}$
    $k$-SS \cite{ye2017optimal} 
    & \cellcolor{OrangeRed!40}$\Theta(d)$ bits 
    & \cellcolor{OrangeRed!40}$\Theta\lp \frac{d}{e^\varepsilon}\rp$ bits 
    \\
\hline %$\vphantom{\Theta \lp \frac{d}{n \min{\lp e, \lp \varepsilon-1\rp, 2\rp}} \rp}$
    HR\cite{acharya2018distributed} 
    & \cellcolor{OrangeRed!40}$\log d$ bits 
    & \cellcolor{OrangeRed!40}$\log d$ bits 
    \\
\hline $\vphantom{\Theta \lp \frac{d}{n \min{\lp e, \lp \varepsilon-1\rp, 2\rp}} \rp}$
    $1$-bit HR\cite{acharya2019communication} 
    & \cellcolor{CornflowerBlue!40} $1$ bit
    & -
    \\
\hline $\vphantom{\Theta \lp \frac{d}{n \min{\lp e, \lp \varepsilon-1\rp, 2\rp}} \rp}$
    Thm.~\ref{thm:dist_estimation}
    & \cellcolor{CornflowerBlue!40}$1$ bit
    & \cellcolor{CornflowerBlue!40}$\Theta\lp \lceil \varepsilon \rceil \rp$ bits 
    \\
\hline
\end{tabular}
    \caption{Comparison between state-of-the-art private distribution estimation schemes.} \label{tbl:dist_compare}
\end{minipage}\hfill
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{./figs/dist_est_acheivability.png}
\captionof{figure}{\cite{acharya2018distributed} is optimal when $b = \log d$, and \cite{acharya2019communication} is optimal when $\varepsilon = O(1)$. Our scheme achieves the lower bound for all regimes.} \label{fig:dist_est_achievability}
\end{minipage}
\end{table}
\fi

